FacePsy: An Open-Source Affective Mobile Sensing System -- Analyzing Facial Behavior and Head Gesture for Depression Detection in Naturalistic Settings

Depression, a prevalent and complex mental health issue affecting millions worldwide, presents significant challenges for detection and monitoring. While facial expressions have shown promise in laboratory settings for identifying depression, their potential in real-world applications remains largely unexplored due to the difficulties in developing efficient mobile systems. In this study, we aim to introduce FacePsy, an open-source mobile sensing system designed to capture affective inferences by analyzing sophisticated features and generating real-time data on facial behavior landmarks, eye movements, and head gestures -- all within the naturalistic context of smartphone usage with 25 participants. Through rigorous development, testing, and optimization, we identified eye-open states, head gestures, smile expressions, and specific Action Units (2, 6, 7, 12, 15, and 17) as significant indicators of depressive episodes (AUROC=81%). Our regression model predicting PHQ-9 scores achieved moderate accuracy, with a Mean Absolute Error of 3.08. Our findings offer valuable insights and implications for enhancing deployable and usable mobile affective sensing systems, ultimately improving mental health monitoring, prediction, and just-in-time adaptive interventions for researchers and developers in healthcare.

==> Section/8_Future_Work.tex <==
\section{Future Work}

==> Section/extra.tex <==
 
\begin{table}[h]
\caption{\label{tab:correlation} Correlation between sensor features and depression binary}


  
\footnotesize
\centering  
    \begin{tabular}{p{3cm}|p{2cm}|p{1cm}|p{3cm}|p{3cm}}
    \toprule
    Top 20 Ranked Feature & Pearson correlation coefficient(r) & p-value & Mean (SD) in depression & Mean (SD) in no-depression \\ 
    \midrule
    % leftEyeOpenProbability\_sum & -0.161 & 0.0 & & \\
    % AU12\_min & 0.115 & 0.0 & & \\
    % AU12\_median & 0.0633 & 0.0 & & \\
    % AU12\_mean & 0.073 & 0.0 & & \\
    % AU12\_q1 & 0.0853 & 0.0 & & \\
    % AU12\_q3 & 0.0527 & 0.0 & & \\
    % AU14\_sum & -0.114 & 0.0 & & \\
    % AU12\_sum & -0.1266 & 0.0 & & \\
    % AU14\_min & 0.0782 & 0.0 & & \\
    % AU14\_q1 & 0.0502 & 0.0 & & \\
    % AU15\_sum & -0.0918 & 0.0 & & \\
    % AU15\_min & 0.0959 & 0.0 & & \\
    % AU15\_median & 0.0819 & 0.0 & & \\
    % AU15\_mean & 0.0795 & 0.0 & & \\
    % AU15\_std & 0.0526 & 0.0 & & \\
    % AU14\_max & -0.0467 & 0.0 & & \\
    % AU15\_q1 & 0.0878 & 0.0 & & \\
    % AU10\_q3 & -0.1049 & 0.0 & & \\
    % AU10\_std & -0.0642 & 0.0 & & \\
    % AU06\_max & -0.1419 & 0.0 & & \\

pir\_left\_min & 0.4184 & 0.0 & 0.1059 (0.0798) & 0.0329 (0.0423) \\
AU15\_q1 & 0.1545 & 0.0 & 0.1635 (0.2105) & 0.0917 (0.1966) \\
pir\_right\_sum & -0.3727 & 0.0 & 5.1043 (6.6566) & 17.2436 (23.3131) \\
AU07\_max & -0.1213 & 0.0 & 0.8285 (0.2335) & 0.8911 (0.2213) \\
pir\_right\_q3 & 0.0949 & 0.0 & 0.3058 (0.2205) & 0.2511 (0.335) \\
AU12\_std & 0.0475 & 0.0 & 0.21 (0.1193) & 0.1966 (0.1439) \\
pir\_right\_std & 0.2835 & 0.0 & 0.1466 (0.104) & 0.0789 (0.1003) \\
pir\_left\_mean & 0.1151 & 0.0 & 0.2487 (0.1746) & 0.1969 (0.2568) \\
AU15\_mean & 0.1429 & 0.0 & 0.2481 (0.2201) & 0.1774 (0.2207) \\
pir\_left\_median & 0.0308 & 0.0 & 0.2162 (0.155) & 0.2027 (0.2741) \\
time\_of\_day & -0.1212 & 0.0 & 12.3003 (6.8897) & 14.1811 (7.0175) \\
pir\_left\_sum & -0.3605 & 0.0 & 5.5458 (6.3728) & 16.6152 (22.0458) \\
pir\_right\_min & 0.4423 & 0.0 & 0.1094 (0.0813) & 0.0303 (0.0395) \\
AU24\_min & 0.0798 & 0.0 & 0.0103 (0.0369) & 0.0042 (0.0243) \\
pir\_left\_q1 & 0.0253 & 0.0002 & 0.1561 (0.1133) & 0.1481 (0.2005) \\
headEulerAngle\_Y\_median & 0.0234 & 0.0007 & -0.049 (7.0394) & -0.4291 (7.9123) \\
leftEyeOpenProbability\_max & -0.0191 & 0.0055 & 0.9367 (0.1574) & 0.9434 (0.1615) \\
AU14\_std & 0.0133 & 0.0536 & 0.2091 (0.1199) & 0.2054 (0.142) \\
pir\_right\_q1 & -0.0098 & 0.156 & 0.159 (0.1138) & 0.1623 (0.2223) \\
pir\_right\_median & -0.0063 & 0.3581 & 0.2179 (0.1563) & 0.2208 (0.303) \\
    \midrule
    \bottomrule
\end{tabular}
\end{table}






\begin{subfigure}{.4\textwidth}
  \centering
  % include second image
  \includegraphics[width=1\linewidth]{Figs/pir_left_sum.png}  
  \caption{\textcolor{purple}{just realized, how come pir\_left\_sum can be greater than 20 at any given data point? there is something weird with the summations. the sampling times may not be consistent. for example, in one of the rows i see pir\_left\_mean=0.27 and pir\_left\_sum= 45. We should probably drop pir sums from analysis. Also, I don't understand why the value dispersions are not continuous. there are only 13 different values pir columns take? }}
  \label{fig:}
\end{subfigure}





\begin{table}
\caption{\textcolor{purple}{not quite matching with SHAP.. headangle\_X correlation is very interesting.. }}
\begin{tabular}{llr}
\toprule
{} & Depression Binary highest correlated features &         r \\
\midrule
0  &                      phq &  0.747846 \\
1  &                      bdi &  0.476106 \\
2  &           panas\_positive & -0.335765 \\
3  &         flowers\_err\_rate & -0.258230 \\
4  &     headEulerAngle\_X\_max & -0.250410 \\
5  &    headEulerAngle\_X\_mean & -0.234935 \\
6  &      headEulerAngle\_X\_q1 & -0.229388 \\
7  &  headEulerAngle\_X\_median & -0.228794 \\
8  &      headEulerAngle\_X\_q3 & -0.227639 \\
9  &     headEulerAngle\_Z\_max & -0.207464 \\
10 &              cma\_valence & -0.202206 \\
11 &      headEulerAngle\_Z\_q3 & -0.197787 \\
12 &     headEulerAngle\_X\_min & -0.197014 \\
13 &                 AU04\_max & -0.196952 \\
14 &    headEulerAngle\_Z\_mean & -0.195197 \\
15 &  headEulerAngle\_Z\_median & -0.194644 \\
16 &             pir\_left\_sum & -0.186315 \\
17 &      headEulerAngle\_Z\_q1 & -0.184908 \\
18 &     headEulerAngle\_X\_sum & -0.173874 \\
19 &                 AU06\_sum & -0.172343 \\
\bottomrule
\end{tabular}
\end{table}





